Efficient Rare Temporal Pattern Mining in Time Series

Time series data from various domains is continuously growing, and extracting and analyzing temporal patterns within these series can provide valuable insights. Temporal pattern mining (TPM) extends traditional pattern mining by incorporating event time intervals into patterns, making them more expressive but also increasing the computational complexity in terms of time and space. One important type of temporal pattern is the rare temporal pattern (RTP), which occurs infrequently but with high confidence. Mining these rare patterns poses several challenges, for example, the low support threshold can lead to a combinatorial explosion and the generation of many irrelevant patterns. To address this, an efficient approach to mine rare temporal patterns is essential. This paper introduces the Rare Temporal Pattern Mining from Time Series (RTPMfTS) method, designed to discover rare temporal patterns. The key contributions of this work are as follows: (1) An end-to-end RTPMfTS process that takes time series data as input and outputs rare temporal patterns. (2) A highly efficient Rare Temporal Pattern Mining (RTPM) algorithm, which leverages optimized data structures for fast event and pattern retrieval, as well as effective pruning techniques to accelerate the mining process. (3) A comprehensive experimental evaluation of RTPM, demonstrating that it outperforms the baseline in both runtime and memory efficiency.

==> refv.tex <==
\bibitem{ahmed2016mining}Akiz Uddin Ahmed, Chowdhury Farhan Ahmed, Md Samiullah, Nahim Adnan, and Carson Kai-Sang Leung. 2016. Mining interesting patterns from uncertain databases. \textit{Information Sciences} 354 (2016).
    
\bibitem{allen}James F Allen. 1983. Maintaining knowledge about temporal intervals. \textit{Commun. ACM} 26 (1983).

\bibitem{batal2012mining}Iyad Batal, Dmitriy Fradkin, James Harrison, Fabian Moerchen, and Milos Hauskrecht. 2012. Mining recent temporal patterns for event detection in multivariate time series data. In \textit{SIGKDD}.

\bibitem{batal2013temporal}Iyad Batal, Hamed Valizadegan, Gregory F Cooper, and Milos Hauskrecht. 2013. A temporal pattern mining approach for classifying electronic health record data. \textit{TIST} 4 (2013).

\bibitem{beckenbach1961introduction}Edwin F Beckenbach, Richard Bellman, and Richard Ernest Bellman. 1961. \textit{An introduction to inequalities}. Technical Report. Mathematical Association of America Washington, DC.

\bibitem{blanchard2005using}Julien Blanchard, Fabrice Guillet, Regis Gras, and Henri Briand. 2005. Using information-theoretic measures to assess association rule interestingness. In \textit{ICDM’05}.

\bibitem{campbell2020temporal}Elizabeth A Campbell, Ellen J Bass, and Aaron J Masino. 2020. Temporal condition pattern mining in large, sparse electronic health record data: A case study in characterizing pediatric asthma. \textit{JAMIA} 27 (2020).

\bibitem{tpminer}Yi-Cheng Chen, Wen-Chih Peng, and Suh-Yin Lee. 2015. Mining Temporal Patterns in Time Interval-Based Data. \textit{TKDE} 27 (2015). 

\bibitem{smartcity}New York City. 2019. NYC OpenData. https://opendata.cityofnewyork.us/

%{\color{blue}\bibitem{zminergit} Lee, Zed and Lindgren, Tony and Papapetrou, Panagiotisu. 2020. Z-Miner. https://github.com/zedshape/zminer}

%{\color{blue}\bibitem{htpgmgit} Van Long, Ho and Nguyen, Ho and Torben Bach, Pedersen. 2021. HTPGM. https://github.com/vanholong/MITPM}

\bibitem{thomas}Thomas M Cover and Joy A Thomas. 2012. \textit{Elements of information theory}. John Wiley \& Sons.

\bibitem{cunjin2015mutual}Xue Cunjin, Song Wanjiao, Qin Lijuan, Dong Qing, and Wen Xiaoyang. 2015. A mutual-information-based mining method for marine abnormal association rules. \textit{Computers \& Geosciences} 76 (2015).

\bibitem{co2} Energi Data Portal. 2021. 
https://www.energidataservice.dk/tso-electricity/co2emis/

\bibitem{pecan}Pecan Street Data. 2016. Pecan Street Dataport. https://www.pecanstreet.org/dataport/

\bibitem{nist}William Healy, Farhad Omar, Lisa Ng, Tania Ullah, William Payne, Brian Dougherty, and A Hunter Fanney. 2018. Net zero energy residential test facility instrumented data. https://pages.nist.gov/netzero/index.html/

\bibitem{ho2020timedelay}Nguyen Ho, Torben Bach Pedersen, Van Long Ho, and Mai Vu. 2020. Efficient Search for Multi-Scale Time Delay Correlations in Big Time Series Data. In 23rd International Conference on Extending Database Technology, EDBT 2020. 37–48.

\bibitem{ho2019icde}Nguyen Ho, Torben Bach Pedersen, Mai Vu, Christophe AN Biscio, et al. 2019. Efficient bottom-up discovery of multi-scale time series correlations using mutual information. In 2019 IEEE 35th International Conference on Data Engineering (ICDE). IEEE, 1734–1737.

\bibitem{ho2019amic}Nguyen Ho, Huy Vo, Mai Vu, and Torben Bach Pedersen. 2019. Amic: An adaptive information theoretic method to identify multi-scale temporal correlations in big time series data. IEEE Transactions on Big Data 7, 1 (2019), 128–146.

\bibitem{ho2016corr} Nguyen Ho, Huy Vo, and Mai Vu. An adaptive information-theoretic approach for identifying temporal correlations in big data sets. In 2016 IEEE International Conference on Big Data (Big Data), pp. 666-675. IEEE, 2016.

\bibitem{ho2022efficientvldb}Van Long Ho, Nguyen Ho, and Torben Bach Pedersen. Efficient temporal pattern mining in big time series using mutual information. In PVLDB, vol. 15, no. 3, 2022.

\bibitem{ho2022seasonal}Van Long Ho, Nguyen Ho, and Torben Bach Pedersen. Mining seasonal temporal patterns in time series. \textit{arXiv preprint arXiv:2206.14604} (2022). https://arxiv.org/abs/2206.14604

\bibitem{ho2020efficient}Van Long Ho, Nguyen Ho, and Torben Bach Pedersen. 2023. Efficient Frequent Temporal Pattern and Rare Temporal Pattern Mining in Big Time Series Using Mutual Information. \textit{arXiv preprint arXiv:2010.03653} (2020). https://arxiv.org/abs/2010.03653

\bibitem{kam2000discovering}Po-shan Kam and Ada Wai-Chee Fu. 2000. Discovering temporal patterns for interval-based events. In \textit{DaWak}.

\bibitem{ke2008correlated}Yiping Ke, James Cheng, and Wilfred Ng. 2008. Correlated pattern mining in quantitative databases. \textit{TODS} 33 (2008).

\bibitem{ho2015datavalue}Thi Thao Nguyen Ho, and Barbara Pernici. A data-value-driven adaptation framework for energy efficiency for data intensive applications in clouds. In 2015 IEEE conference on technologies for sustainability (SusTech), pp. 47-52. IEEE, 2015.

%\newpage

\bibitem{ho2017improving}Thi Thao Nguyen Ho, Marco Gribaudo, and Barbara Pernici. "Improving energy efficiency for transactional workloads in cloud environments." In Proceedings of the Eighth International Conference on Future Energy Systems, pp. 290-295. 2017.

\bibitem{energy2016}Thi Thao Nguyen Ho, Marco Gribaudo, and Barbara Pernici. "Characterizing energy per job in cloud applications." Electronics 5, no. 4 (2016): 90.

\bibitem{energy2014}Macro Gribaudo, Thi Thao Nguyen Ho, Barbara Pernici, and Giuseppe Serazzi. "Analysis of the influence of application deployment on energy consumption." In International Workshop on Energy Efficient Data Centers, pp. 87-101. Springer, Cham, 2014.

\bibitem{ukdale}Jack Kelly and William Knottenbelt. 2015. The UK-DALE dataset, domestic appliance-level electricity demand and whole-house demand from five UK homes. \textit{Scientific Data} (2015).

\bibitem{lee2003comine}Young-Koo Lee, Won-Young Kim, Y Dora Cai, and Jiawei Han. 2003. CoMine: Efficient Mining of Correlated Patterns. In \textit{ICDM}.

\bibitem{lee2020z}Zed Lee, Tony Lindgren, and Panagiotis Papapetrou. 2020. Z-Miner: An Efficient Method for Mining Frequent Arrangements of Event Intervals. In \textit{Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining}. 524–534.

\bibitem{lin2003symbolic}Jessica Lin, Eamonn Keogh, Stefano Lonardi, and Bill Chiu. 2003. A symbolic representation of time series, with implications for streaming algorithms. In \textit{Proceedings of the 8th ACM SIGMOD workshop on Research issues in data mining and knowledge discovery}. 2–11.

\bibitem{megalooikonomou2005multiresolution}Vasileios Megalooikonomou, Qiang Wang, Guo Li, and Christos Faloutsos. 2005. A multiresolution symbolic representation of time series. In \textit{21st International Conference on Data Engineering (ICDE’05)}. IEEE, 668–679.

\bibitem{morchen2007unsupervised}Fabian Mörchen. 2007. Unsupervised pattern mining from symbolic temporal data. \textit{ACM SIGKDD Explorations Newsletter} 9, 1 (2007), 41–55.

\bibitem{moskovitch2015fast}Robert Moskovitch and Yuval Shahar. 2015. Fast time intervals mining using the transitivity of temporal relations. \textit{KAIS} 42 (2015).

\bibitem{neidle2018new}Carol Neidle, Augustine Opoku, Gregory Dimitriadis, and Dimitris Metaxas. 2018. NEW Shared \& Interconnected ASL Resources: SignStream® 3 Software; DAI 2 for Web Access to Linguistically Annotated Video Corpora; and a Sign Bank. In \textit{8th Workshop on the Representation and Processing of Sign Languages: Involving the Language Community, Miyazaki, Language Resources and Evaluation Conference
    2018}.

\bibitem{omiecinski2003alternative}Edward R Omiecinski. 2003. Alternative interest measures for mining associations in databases. \textit{IEEE Transactions on Knowledge and Data Engineering 15}, 1 (2003),
57–69.

\bibitem{hdfs}Panagiotis Papapetrou, George Kollios, Stan Sclaroff, and Dimitrios Gunopulos. 2009. Mining frequent arrangements of temporal intervals. \textit{KAIS} 21 (2009).

\bibitem{ieminer}Dhaval Patel, Wynne Hsu, and Mong Li Lee. 2008. Mining relationships among interval-based events for classification. In \textit{SIGMOD}.

\bibitem{sharma2018stipa}Amit Kumar Sharma and Dhaval Patel. 2018. Stipa: A memory efficient technique for interval pattern discovery. In \textit{2018 IEEE International Conference on Big Data (Big Data)}. IEEE, 1767–1776.

\bibitem{wang2020mining}Jun-Zhe Wang, Yi-Cheng Chen, Wen-Yueh Shih, Lin Yang, Yu-Shao Liu, and Jiun-Long Huang. 2020. Mining High-utility Temporal Patterns on Time Interval–based Data. \textit{ACM Transactions on Intelligent Systems and Technology (TIST)} 11, 4 (2020), 1–31.

\bibitem{wu2007mining}Shin-Yi Wu and Yen-Liang Chen. 2007. Mining nonambiguous temporal patterns for interval-based events. \textit{TKDE} 19 (2007).

\bibitem{yao2003information}YY Yao. 2003. Information-theoretic measures for knowledge discovery and data mining. In \textit{Entropy measures, maximum entropy principle and emerging applications}. 115–136.

\bibitem{torp2019traveltime} Torp K., Andersen O., Thomsen C. (2020) Travel-Time Computation Based on GPS Data. In: Kutsche RD., Zimányi E. (eds) Big Data Management and Analytics. eBISS 2019. Lecture Notes in Business Information Processing, vol 390. Springer, Cham. https://doi.org/10.1007/978-3-030-61627-4\_4.

\bibitem{corless1996lambertw} RobertMCorless, Gaston H Gonnet, David EG Hare, David J Jeffrey, and Donald E
Knuth. 1996. On the LambertW function. Advances in Computational mathematics 5, 1 (1996), 329–359.

\bibitem{huang2012rarepatterndatastream} Huang, David, Yun Sing Koh, and Gillian Dobbie. "Rare pattern mining on data streams." International Conference on Data Warehousing and Knowledge Discovery. Springer, Berlin, Heidelberg, 2012.

\bibitem{gao2017motif} Gao, Yifeng, and Jessica Lin. "Efficient discovery of time series motifs with large length range in million scale time series." 2017 IEEE International Conference on Data Mining (ICDM). IEEE, 2017.

\bibitem{begum2014raremotif} Begum, Nurjahan, and Eamonn Keogh. "Rare time series motif discovery from unbounded streams." Proceedings of the VLDB Endowment 8.2 (2014): 149-160.

\bibitem{li2022asso} Li, Yun, and Saihua Cai. "Detecting Outliers in Data Streams Based on Minimum Rare Pattern Mining and Pattern Matching." Information Technology and Control 51.2 (2022): 268-282.

\bibitem{cui2022asso} Cui, Yanling, et al. "FRI-miner: fuzzy rare itemset mining." Applied Intelligence 52.3 (2022): 3387-3402.

\bibitem{ji2021asso} Ji, Yi, and Yukio Ohsawa. "Mining Frequent and Rare Itemsets With Weighted Supports Using Additive Neural Itemset Embedding." 2021 International Joint Conference on Neural Networks (IJCNN). IEEE, 2021.

\bibitem{cai2021asso} Cai, Saihua, et al. "An efficient anomaly detection method for uncertain data based on minimal rare patterns with the consideration of anti-monotonic constraints." Information Sciences 580 (2021): 620-642.

\bibitem{ali2021asso} Alipourchavary, Elaheh, Sarah M. Erfani, and Christopher Leckie. "Mining Rare Recurring Events in Network Traffic using Second Order Contrast Patterns." 2021 International Joint Conference on Neural Networks (IJCNN). IEEE, 2021.

\bibitem{bouasker2020asso} Bouasker, Souad, et al. "Pregnancy Associated Breast Cancer gene expressions: new insights on their regulation based on Rare Correlated Patterns." IEEE/ACM Transactions on Computational Biology and Bioinformatics 18.3 (2020): 1035-1048.

\bibitem{borah2020asso} Borah, Anindita, and Bhabesh Nath. "Rare association rule mining from incremental databases." Pattern Analysis and Applications 23.1 (2020): 113-134.

\bibitem{fournier2020asso} Fournier-Viger, Philippe, et al. "Discovering rare correlated periodic patterns in multiple sequences." Data \& Knowledge Engineering 126 (2020): 101733.

\bibitem{biswas2019asso} Biswas, S., \& Mondal, K. C. (2019). Dynamic FP tree based rare pattern mining using multiple item supports constraints. In Computational Intelligence, Communications, and Business Analytics: Second International Conference, CICBA 2018, Kalyani, India, July 27–28, 2018, Revised Selected Papers, Part II 2 (pp. 291-305). Springer Singapore.

\bibitem{piri2018asso} Piri, Saeed, et al. "Development of a new metric to identify rare patterns in association analysis: The case of analyzing diabetes complications." Expert Systems with Applications 94 (2018): 112-125.

\bibitem{rahman2019sequential} Rahman, Anisur. Rare sequential pattern mining of critical infrastructure control logs for anomaly detection. Diss. Queensland University of Technology, 2019.

\bibitem{iqbal2019sequential} Iqbal, Mohammad, et al. "Mining Non-Zero-Rare Sequential Patterns On Activity Recognition." Jurnal Matematika MANTIK 5.1 (2019): 1-9.

\bibitem{samed2017sequential} Samet, Ahmed, Thomas Guyet, and Benjamin Negrevergne. "Mining rare sequential patterns with ASP." (2017).

\bibitem{rahman2016sequential} Rahman, Anisur, et al. "Finding anomalies in SCADA logs using rare sequential pattern mining." International Conference on Network and System Security. Springer, Cham, 2016.

\bibitem{zhu2016sequential} Zhu, Jiaqi, et al. "Mining user-aware rare sequential topic patterns in document streams." IEEE Transactions on Knowledge and Data Engineering 28.7 (2016): 1790-1804.

\bibitem{ou2016sequential} Ouyang, Weimin. "Mining Rare Sequential Patterns in Large Transaction Databases." 2016 International Conference on Computer Science and Electronic Technology. Atlantis Press, 2016.
